Rank It, Then Ask It: Input Reranking for Maximizing the Performance of LLMs on Symmetric Tasks

Large language models (LLMs) have quickly emerged as practical and versatile tools that provide new solutions for a wide range of domains. In this paper, we consider the application of LLMs on symmetric tasks where a query is asked on an (unordered) bag of elements. Examples of such tasks include answering aggregate queries on a database table. In general, when the bag contains a large number of elements, LLMs tend to overlook some elements, leading to challenges in generating accurate responses to the query. LLMs receive their inputs as ordered sequences. However, in this problem, we leverage the fact that the symmetric input is not ordered, and reordering should not affect the LLM's response. Observing that LLMs are less likely to miss elements at certain positions of the input, we introduce the problem of LLM input reranking: to find a ranking of the input that maximizes the LLM's accuracy for the given query without making explicit assumptions about the query. Finding the optimal ranking requires identifying (i) the relevance of each input element for answering the query and (ii) the importance of each rank position for the LLM's attention. We develop algorithms for estimating these values efficiently utilizing a helper LLM. We conduct comprehensive experiments on different synthetic and real datasets to validate our proposal and to evaluate the effectiveness of our proposed algorithms. Our experiments confirm that our reranking approach improves the accuracy of the LLMs on symmetric tasks by up to $99\%$ proximity to the optimum upper bound.

==> bios.tex <==
\section{Short Bios}

\noindent
{\bf Abolfazl Asudeh} is an assistant professor of Computer Science at the University of Illinois Chicago and the director of Innovative Data Exploration Laboratory (InDeX Lab). He is a VLDB Ambassador, the VLDB Endowment’s Liaison to NSF, and a regular PC member of Database flagship venues. His research spans to different aspects of Data Management, for which he designs efficient, accurate, and scalable algorithmic solutions. Responsible Data Management, including Data Equity Systems, Algorithmic Fairness, and Data-centric AI, is his major focus in research.


\smallskip
\noindent\textbf{Sainyam Galhotra} is an Assistant Professor in the Computer Science department at Cornell University. Before that, he was a Computing Innovation Postdoctoral Fellow at the University of Chicago. The goal of his research is to lay the foundation of responsible data science, that enables efficient development and deployment of trustworthy data analytics applications. His research has combined techniques from Data Management, Probabilistic Methods, Causal Inference, Machine Learning, and Software Engineering. He received his Ph.D. from the University of Massachusetts Amherst. He is a recipient of the Best Paper Award in FSE 2017 and the Most Reproducible Paper Award in SIGMOD 2017 and 2018. He is a DAAD AInet Fellow, and the first recipient of the Krithi Ramamritham Award at UMass for contribution to database research.


\smallskip
\noindent\textbf{Amir Gilad} is an Assistant Professor at the Hebrew University of Jerusalem’s School of Computer Science and Engineering. 
His research focuses on data analysis, data management, causal analysis, and differential privacy. He is working on the development of tools and algorithms that aim to assist users in understanding and gaining insights into data through explanations and causal analysis. He is also studying the privacy implications of providing such explanations.
He is a recipient of the 2017 VLDB Best Paper Award, the 2018 SIGMOD Research Highlight Award, and the 2019 Google Ph.D. Fellowship in Structured Data and Database Management. 
Before joining The Hebrew University, he was a postdoctoral researcher in the Database Group at Duke University,  and received his Ph.D in Computer Science from Tel Aviv University.

\smallskip
\noindent\textbf{Babak Salimi} is an Assistant Professor at the Halıcıoğlu Data Science Institute, also holding an affiliation with the Department of Computer Science and Engineering at the University of California, San Diego. Before his appointment at UCSD, he was engaged as a postdoctoral research associate at the University of Washington, contributing to the UW Database Group under the guidance of Prof. Dan Suciu. His academic journey includes earning a Ph.D. in 2016 from Carleton University, where he was advised by Prof. Leopoldo Bertossi. Salimi's notable recognitions include the Postdoc Research Award at the University of Washington in 2017, a Best Demonstration Paper Award at VLDB in 2018, a Best Paper Award at SIGMOD in 2019, and a Research Highlight Award at SIGMOD in 2020..

\smallskip
\noindent\textbf{Brit Youngmann} is an Assistant Professor at the Technion’s Faculty of Computer Science. 
Her research focuses on data management, causal reasoning, and responsible data management. She is developing automatized data tools to facilitate data analysis performed by scientists to accelerate scientific discoveries. Her research draws on ideas from data management and causal reasoning, making them practical for goal-oriented scientists working with real-life datasets.
She is the recipient of several awards, including the data science fellowship for outstanding Ph.D. students of the planning and budgeting committee of the Israeli council for higher education, and the Schmidt postdoctoral award for women in mathematical and computing sciences.  
Before joining The Technnion, she was a postdoctoral researcher in the Data System Group at MIT, and received her Ph.D in Computer Science from Tel Aviv University.

